GLITTER: An AI-assisted Platform for Material-Grounded Asynchronous Discussion in Flipped Learning

Flipped classrooms promote active learning by having students engage with materials independently before class, allowing in-class time for collaborative problem-solving. During this pre-class phase, asynchronous online discussions help students build knowledge and clarify concepts with peers. However, it remains difficult to engage with temporally dispersed peer contributions, connect discussions with static learning materials, and prepare for in-class sessions based on their self-learning outcome. Our formative study identified cognitive challenges students encounter, including navigation barriers, reflection gaps, and contribution difficulty and anxiety. We present GLITTER, an AI-assisted discussion platform for pre-class learning in flipped classrooms. GLITTER helps students identify posts with shared conceptual dimensions, scaffold knowledge integration through conceptual blending, and enhance metacognition via personalized reflection reports. A lab study within subjects (n = 12) demonstrates that GLITTER improves discussion engagement, sparks new ideas, supports reflection, and increases preparedness for in-class activities.

==> sections/_scratchpad.tex <==
% April's Attempt of the Abstract

Monitoring in-class programming exercises offers real-time insights, helping instructors quickly identify struggling students or common misconceptions.
However, this becomes challenging when exercises involve non-linear solution paths with nested substeps, where some steps are interdependent and others independent (e.g., in web programming).
We introduce SPARK, a coding exercise monitoring dashboard designed to address these challenges.
SPARK allows instructors to flexibly group substeps into checkpoints based on exercise requirements, suggests automated testing for these checkpoints, and generates visualizations to track progress.
It also enables inspection of intermediate outputs at each checkpoint, providing deeper insights into solution variations.
In addition to the design of SPARK, we constructed a dataset of 30 minutes keystroke coding data from N=20 learners solving two web programming exercises, collected from a custom code editor extension.
We also provided empirical insights into the perceived usefulness of SPARK through a within-subjects evaluation with 16 instructors and teaching assistants.



